AttenMIA: LLM Membership Inference Attack through Attention Signals

Large Language Models (LLMs) are increasingly deployed to enable or improve a multitude of real-world applications. Given the large size of their training data sets, their tendency to memorize training data raises serious privacy and intellectual property concerns. A key threat is the membership inference attack (MIA), which aims to determine whether a given sample was included in the model's training set. Existing MIAs for LLMs rely primarily on output confidence scores or embedding-based features, but these signals are often brittle, leading to limited attack success. We introduce AttenMIA, a new MIA framework that exploits self-attention patterns inside the transformer model to infer membership. Attention controls the information flow within the transformer, exposing different patterns for memorization that can be used to identify members of the dataset. Our method uses information from attention heads across layers and combines them with perturbation-based divergence metrics to train an effective MIA classifier. Using extensive experiments on open-source models including LLaMA-2, Pythia, and Opt models, we show that attention-based features consistently outperform baselines, particularly under the important low-false-positive metric (e.g., achieving up to 0.996 ROC AUC & 87.9% TPR@1%FPR on the WikiMIA-32 benchmark with Llama2-13b). We show that attention signals generalize across datasets and architectures, and provide a layer- and head-level analysis of where membership leakage is most pronounced. We also show that using AttenMIA to replace other membership inference attacks in a data extraction framework results in training data extraction attacks that outperform the state of the art. Our findings reveal that attention mechanisms, originally introduced to enhance interpretability, can inadvertently amplify privacy risks in LLMs, underscoring the need for new defenses.

==> sections/ablation_study.tex <==
%\section{Ablation Study}
%\label{sec: Ablation_Study}

\noindent \textbf{Impact of input perturbation strategies.} 
We next study how different perturbation strategies influence attack performance. 
We evaluate three perturbations: (i) non-member prefix insertion, (ii) token dropping, and (iii) token replacement. These perturbations simulate natural variations in phrasing and test the stability of attention-based membership signals.
As shown in Table~\ref{tab:ablation_results_perturbations}, all three perturbation types yield comparable performance individually, and combining them produces the strongest results.


\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{9}{c}{} \\
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{2}{c}{\textbf{Wikipedia}} &
\multicolumn{2}{c}{\textbf{GitHub}} &
\multicolumn{2}{c}{\textbf{Pile CC}} &
\multicolumn{2}{c}{\textbf{PubMed Central}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR \\
\midrule

AttenMIA (Non-Member Prefix)  & 0.61 & 11.5 & 0.92 & 73.6 & 0.60 & 6.5 & 0.86 & 24.5  \\
AttenMIA (Dropping Tokens)  & 0.62 & 11.5 & 0.92 & 74.3 & 0.59 & 5.1 & 0.86 & 27.5  \\
AttenMIA (Replacing Tokens)  & 0.62 & 11.6 & 0.92 & 72.2 & 0.59 & 3.7 & 0.86 & 28.7    \\

\midrule
\multicolumn{9}{c}{} \\
\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{2}{c}{\textbf{arXiv}} &
\multicolumn{2}{c}{\textbf{DM Math}} &
\multicolumn{2}{c}{\textbf{HackerNews}} &
\multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR & ROC AUC & TPR@1\%FPR  \\
\midrule


AttenMIA (Non-Member Prefix)  & 0.82 & 33.4 & 0.96 & 89.6 & 0.62 & 6.6 & 0.77 & 35.1  \\
AttenMIA (Dropping Tokens)  & 0.82 & 31.6 & 0.96 & 90.6 & 0.61 & 10.5 & 0.77 & 35.9  \\
AttenMIA (Replacing Tokens)  & 0.81 & 36.2 & 0.96 & 89.5 & 0.60 & 9.0 & 0.77 & 35.8  \\

\bottomrule
\end{tabular}
}
\caption{ROC AUC scores and TPR@1\%FPR of AttenMIA using individual perturbations. We experiment on the Pythia-1.4B model and different subsets of the MIMIR benchmark.}
\label{tab:ablation_results_perturbations}
\end{table*}


% ****************************************************************************************


\noindent \textbf{Analyzing the role of different layers in MIA.}
To study where memorization resides within the transformer, we analyze how different transformer layers contribute to membership inference. Using the perturbed attention features of the Pythia-1.4B model (24 layers) on the PubMed Central subset, we consider three settings: (i) features from a single layer, (ii) features grouped into lower, middle, and upper segments, and (iii) all layers combined.

Figure~\ref{fig:layer_analysis} shows that every layer contains meaningful membership information, though individual layers vary moderately in discriminative strength. Aggregating features within layer groups consistently improves performance over single layers, and using all 24 layers yields the highest ROC AUC. This suggests that memorization is not localized, and it is distributed across the layers and best captured when features from multiple depths are integrated. \\ 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{img/layer_analysis1.pdf}
    \caption{ROC AUC of AttenMIA using perturbed features from different layers of Pythia-1.4B on the PubMed Central dataset. We compare individual layers (blue bars), grouped layers (orange bars), and all layers combined. Results show that every layer contributes useful membership information, with performance improving when aggregating across groups, and peaking when all layers are used together.}
    \label{fig:layer_analysis}
\end{figure}





% ****************************************************************************************

\noindent \textbf{Effect of sequence length on AttenMIA.}  
We examine how input sequence length influences membership inference. Using WikiMIA, we evaluate Pythia-6.9B, Llama2-13B, and NeoX-20B under two feature families, Transitional Features and Perturbed Features, across lengths 32, 64, and 128 tokens. Figure~\ref{fig:length_effect} represents two consistent trends.

First, shorter sequences produce stronger membership signals, especially for TPR@1\%FPR. With transitional features, NeoX-20B achieves nearly 100\% ROC AUC and TPR@1\%FPR at length 32; performance then gradually decreases as the sequence length increases. A similar pattern appears for perturbed features. This suggests that memorization signals are more concentrated and easier to extract in shorter contexts, whereas longer contexts introduce noise that obscures membership-specific patterns.

Second, despite this degradation, \textsc{AttenMIA} remains consistently effective across all models and sequence lengths, outperforming baseline attacks throughout (see Section~\ref{sec:main_results}). The larger performance drop in TPR@1\%FPR compared to AUC further indicates that the low-FPR setting is more sensitive to long contexts, an important consideration for real-world auditing.

% These findings underscore the importance of considering input length when auditing LLMs for memorization, as models may appear more robust when evaluated on longer sequences, even though shorter sequences expose stronger privacy risks.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{img/length_effect.pdf}
    \caption{Effect of sequence length on AttenMIA performance. We plot ROC AUC (left column) and TPR@1\%FPR (right column) for Pythia-6.9B, LLaMA-13B, and NeoX-20B under both transitional and perturbed feature settings. Shorter sequences yield stronger membership signals, while performance degrades at longer lengths.}
    \label{fig:length_effect}
\end{figure}

==> sections/defenses.tex <==
\section{AttenMIA against Defenses}



% \subsection{MemGuard} 
% MemGuard~\cite{jia2019memguard} is a defense strategy that mitigates membership inference risk by masking confidence scores. It injects carefully crafted noise into the probability vectors output by the target model, effectively transforming them into adversarial examples that force attackers toward random guessing. While MemGuard has demonstrated strong protection against logits-based MIAs, its effectiveness is limited against approaches that do not rely directly on model probabilities. In particular, since our perturbation-based features approximate distributions via semantic shifts rather than raw output logits, the crafted noise does not degrade attack performance. Importantly, because MemGuard preserves the predicted label to maintain utility, semantic-based attacks such as ours can still recover meaningful membership signals despite the defense.





\noindent \textbf{Training Data Deduplication. }
Prior work suggests that removing duplicated text from pre-training corpora can reduce memorization and thereby mitigate membership inference risks in LLMs~\cite{kandpal2022deduplicating, lee2021deduplicating}. The intuition is that duplicated data inflates memorization, so removing it should reduce vulnerability. This approach is generally more efficient than training-based defenses such as differential privacy, and it has been viewed as a practical mitigation strategy.

To evaluate whether deduplication weakens the signals exploited by \textsc{AttenMIA}, we test it on the Pythia-dedup family~\cite{biderman2023pythia}, which matches Pythia in architecture and size but is trained on a deduplicated version of the Pile. Table~\ref{tab:dedup_results_AUC} reports ROC AUC on the GitHub and HackerNews subsets across multiple model scales. Deduplication yields only negligible differences in attack performance, typically within 0.00–0.03 AUC. For instance, \textit{AttenMIA} achieves 0.99 ROC AUC on GitHub for all scales, regardless of deduplication. HackerNews shows a similarly minimal change, remaining around 0.70–0.71 ROC AUC.

These results indicate that deduplication alone is insufficient to meaningfully reduce membership signals exploited by AttenMIA. Our results highlight the need for stronger or more principled defenses beyond deduplication to mitigate membership leakage in modern LLMs. Additional experiments are provided in Appendix~\ref{appendix: DEDUPLICATION}.




\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\multicolumn{13}{c}{} \\
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{GitHub}} &
\multicolumn{3}{c}{\textbf{HackerNews}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
& Pythia-1.4b & Pythia-2.8b & Pythia-6.9b & Pythia-1.4b & Pythia-2.8b & Pythia-6.9b  \\
\midrule

PPL attack  & 0.86 (0.00) & 0.87 (0.00) & 0.87 (-0.01) & 0.59 (0.00) & 0.60 (0.00) & 0.59 (-0.01)  \\

reference attack & 0.62 (-0.03) & 0.64 (-0.01) & 0.61 (-0.03) & 0.52 (0.00)  & 0.53 (0.00) & 0.52 (0.00)  \\

zlib attack & 0.85 (0.00) & 0.86 (0.00) & 0.86 (-0.01) & 0.59 (0.00) & 0.59 (0.00) & 0.59 (0.00) \\

neighborhood attack & 0.83 (0.00) & 0.82 (0.00) & 0.82 (-0.02) & 0.54 (0.00) & 0.54 (0.00) & 0.54 (-0.01)  \\

MIN-K\% PROB & 0.85 (-0.01) & 0.86 (0.00) & 0.87 (-0.01) & 0.56 (-0.01) & 0.58 (0.00) & 0.56 (-0.02)  \\

PETAL & 0.85 (0.00) & 0.86 (0.00) & 0.87 (-0.01) & 0.56 (-0.01) & 0.58 (0.00) & 0.56 (-0.02)  \\

AttenMIA (Raw Features)  & 0.90 (+0.02) & 0.92 (-0.01) & 0.88 (-0.01) & 0.61 (-0.01) & 0.59 (0.00) & 0.61 (+0.02)  \\
AttenMIA (Perturbed Features) & 0.99 (0.00)  & 0.99 (0.00) & 0.99 (-0.01) & 0.70 (0.00) & 0.71 (-0.01) & 0.71 (-0.01) \\

\bottomrule
\end{tabular}
}
\caption{ROC AUC results of AttenMIA and baselines on deduplicated Pythia models. Numbers in parentheses denote the change relative to the non-deduplicated Pythia counterparts. Results show that deduplication has a negligible impact on MIA effectiveness.}
\label{tab:dedup_results_AUC}
\end{table*}

